Panoptic Image Annotation with a Collaborative Assistant

This paper aims to reduce the time to annotate images for panoptic segmentation, which requires annotating segmentation masks and class labels for all object instances and stuff regions. We formulate our approach as a collaborative process between an annotator and an automated assistant who take turns to jointly annotate an image using a predefined pool of segments. Actions performed by the annotator serve as a strong contextual signal. The assistant intelligently reacts to this signal by annotating other parts of the image on its own, which reduces the amount of work required by the annotator. We perform thorough experiments on the COCO panoptic dataset, both in simulation and with human annotators. These demonstrate that our approach is significantly faster than the recent machine-assisted interface of [4], and 2.4x to 5x faster than manual polygon drawing. Finally, we show on ADE20k that our method can be used to efficiently annotate new datasets, bootstrapping from a very small amount of annotated data.

==> context_model.tex <==
The structure of our context model is schematically shown on Fig.~\ref{}. The model independently
updates class probabilities of each proposal segment given the fixed set $X_{fix}$. \footnote{Our
  formulation assumes that elements in the proposal set $X_{p}$ are independent of each other given
  the fixed set $X_{fix}$. We leave the extension that jointly models all segments for a future
  work. A possible avenue towards jointly modeling all segments would be build on the
  graph-convolutional networks as in \cite{}.}. 

Our starting point for building the context model is a building block in Fig.~\ref{}. The model takes
segment features $\xprop^j$ and computes incremental updates to these features using a small fully
connected neural network $\Eprop$. This is similar to a module in the ResNet network and has been
previously used in the literature \cite{carreira16cvpr}. 

To incorporate information from the fixed set we extend this model with additional network that
first computes fixed size representation vector that captures relative features between a particular
fixed segment $\xfix$ and a given proposal segment $\xprop$. The embedding is implemented using
subnetwork $\Efix$ show on Fig.~\ref{}. 

Intuitively the objective of $\Efix$ is to extract information from the spatial distribution of
segment pairs within the image that is useful for predicting class distribution of the proposal
segment. In our implementation we first apply several fully connected layers to each of the feature
type of each segment and then combine all the features in the final layer. 

We apply average pulling to merge the outputs of $\Efix$ components corresponding to each fixed
segment and then combine the result with the features of the proposal segment generated by $\Eprop$
to incrementally update the class probabilities. 

\mypar{Discussion.} Useful properties of this model:
(1) incremental updates, (2) supports variable cardinality of the fixed set, and (3) is invariant to
ordering in which elements are added to the fixed set. Limitations: (1) pairwise only and (2)
assumes proposal segments are independent and (3) does not perform reasoning on which proposal
should be placed first in the image (follows from the assumption of independence of the proposal
segments) and in particular does not learn non-maximum suppression. We will address limitations in
the future work.





==> fig_assistant_actions.tex <==




\bgroup
\tabcolsep 0.5pt

\begin{figure}[t]
    \centering
    \begin{tabular}{cccc}
      \includegraphics[width=0.25\textwidth]{figures/images/000093_110721_image.png}&
      \includegraphics[width=0.25\textwidth]{figures/images/000093_110721_human.png}&
      \includegraphics[width=0.25\textwidth]{figures/images/000093_110721_assistant_highlights.png}&
      \includegraphics[width=0.25\textwidth]{figures/images/000093_110721_gt.png}\\
      \scriptsize{(a) input image}  & \scriptsize{(b) the annotator changes} &
      \scriptsize{(c) the assistant reacts} & \scriptsize{(d) ground-truth}\vspace{-.15cm}\\
      & \scriptsize{\emph{road} to \emph{pavement}} & \scriptsize{by changing labels} & \vspace{0.2cm}\\
      \includegraphics[width=0.25\textwidth]{figures/images/table_scene_new_labels/table_scene_img_crop.png}&
      \includegraphics[width=0.25\textwidth]{figures/images/table_scene_new_labels/000401_human.png}&
      \includegraphics[width=0.25\textwidth]{figures/images/table_scene_new_labels/000401_assistant_highlights.png}&
      \includegraphics[width=0.25\textwidth]{figures/images/table_scene_new_labels/000401_142620.png}\\
      \scriptsize{(e) input image} & \scriptsize{(f) the annotator changes} &
      \scriptsize{(g) the assistant reacts} & \scriptsize{(h) ground-truth}\vspace{-.15cm}\\
      & \scriptsize{\emph{cup} to \emph{bowl}} & \scriptsize{by adding segments} & \\
    \end{tabular}
    \caption{Example of the collaborative annotation process. Given an input image, the human annotator and the automated assistant
      carry out actions in turn. Based on the current annotation, the annotator performs one action (highlighted in red). Then the assistant reacts with by changing labels (in blue) and adding segments (in green). For comparison we show the ground-truth panoptic segmentation.}
    \label{fig:actionexample}
\end{figure}
\egroup



==> fig_fix1.tex <==
\bgroup
\tabcolsep 0.5pt
\begin{figure}[t]
\vspace{-0.5cm}
    \centering
    \begin{tabular}{cc}
      \includegraphics[width=0.5\linewidth]{figures/examples_fix1/airplane_image_fix_none_dot}&
      \includegraphics[width=0.5\linewidth]{figures/examples_fix1/airplane_image_fix_train_dot}\vspace{-0.1cm}\\
      \scriptsize{(a)} & \scriptsize{(b)}\vspace{0.2cm}\\
      \includegraphics[width=0.5\linewidth]{figures/examples_fix1/food_image_fix_none_dot}&
      \includegraphics[width=0.5\linewidth]{figures/examples_fix1/food_image_fix_tennis_dot}\vspace{-0.1cm}\\
      \scriptsize{(c)} & \scriptsize{(d)}\vspace{0.2cm}\\
    \end{tabular}
    \caption{Original class labels (a, b) and updated labels based on the generic context 
      model (b, d). In each case the fixed set if composed of a single segment marked with a yellow
      dot. For demonstration purposes we deliberately set the label of the fixed segments to
      ``train'' (top row) and ``tennis racket'' (bottom row).}
    \label{fig:examples_fix1}
\end{figure}
\egroup



==> fig_proposal_active_fixed.tex <==

\begin{figure}[t]
  \vspace{-0.0cm}
    \centering
      \includegraphics[width=\linewidth]{figures/proposal_set_example}\\
      \caption{The \emph{proposal set}, \emph{active set} and \emph{fixed set}. The \emph{proposal set} is the complete segment pool created by Mask-RCNN (only a few shown for clarity). The \emph{active set} defines the current annotation (segments 3, 5, 7 here). The \emph{fixed set} contains segments which were modified or added by the annotator and are considered to be ground-truth (only segment 7 here). %
      }
    \label{fig:illustration_proposal_set}
\end{figure}









==> fig_results_context_model.tex <==

\begin{figure}[t]
    \centering
    \vspace{-.0cm}
    \includegraphics[width=0.6\linewidth]{figures/plot_change_label_60k.png}
    \caption{Class label accuracy delivered by our context model (red, blue) as a function of the number of fixed segments given to it. The Mask-RCNN baseline (dashed black) represents the starting point without context model. Note that for $\Kfix = 0$ the accuracy of the ensemble model is higher than the baseline due to local score pooling (Eq.~\eqref{eq:local_pooling}).}
    \label{fig:change_label_results60k}
    \vspace{-.3cm}
\end{figure}


